Optimized Vectorizing of Building Structures with Switch: High-Efficiency Convolutional Channel-Switch Hybridization Strategy

The building planar graph reconstruction, a.k.a. footprint reconstruction, which lies in the domain of computer vision and geoinformatics, has been long afflicted with the challenge of redundant parameters in conventional convolutional models. Therefore, in this letter, we proposed an advanced and adaptive shift architecture, namely the Switch operator, which incorporates non-exponential growth parameters while retaining analogous functionalities to integrate local feature spatial information, resembling a high-dimensional convolution operation. The Switch operator, cross-channel operation, architecture implements the XOR operation to alternately exchange adjacent or diagonal features, and then blends alternating channels through a 1x1 convolution operation to consolidate information from different channels. The SwitchNN architecture, on the other hand, incorporates a group-based parameter-sharing mechanism inspired by the convolutional neural network process and thereby significantly reducing the number of parameters. We validated our proposed approach through experiments on the SpaceNet corpus, a publicly available dataset annotated with 2,001 buildings across the cities of Los Angeles, Las Vegas, and Paris. Our results demonstrate the effectiveness of this innovative architecture in building planar graph reconstruction from 2D building images.

==> section/2-related.tex <==
\section{Related Works}
\label{ch:review}
There are generally two approaches to extracting the building boundary edges: the subspace search method~\cite{nauata2020vectorizing}, and the pixel-based method~\cite{abdellatif2021combining}, and both of them rely on deep learning models.
\par
The subspace search method typically involves searching for the optimal solution within a subspace of edges. This method requires defining an objective function and iteratively optimizing it to obtain the most accurate boundaries. However, this method can be computationally expensive, and the accuracy of the results depends heavily on the chosen objective function.
\par
In contrast, the pixel-based method~\cite{abdellatif2021combining} leverages purely deep learning to automatically learn the optimal boundary detection algorithm from a large amount of annotated training data. This method is typically more efficient than the subspace search method and can achieve high accuracy even in complex environments. However, the pixel-based method requires a large amount of labeled training data and may suffer from overfitting if the data is not representative of the actual target domain.
\par
\subsection{DL Based with Subspace Search}
Subspace search, always combined with typology, is a method for edge detection and wireframe parsing that involves searching for the optimal subspace of the image space. It can achieve high accuracy in edge detection, especially for objects with simple geometric shapes such as straight lines or circles. However, subspace search also has limitations, such as its sensitivity to noise and occlusions in the input image, and its inability to handle complex wireframes with non-linear shapes.
\par
Nelson Nauata and Yasutaka Furukawa ~\cite{nauata2020vectorizing} proposed a novel algorithm for planar graph reconstruction of world buildings, which combines CNNs with typology-based methods. The algorithm consists of two main components: primitive detection and relationship inference, and planar graph assembly.
%
For the primitive detection and relationship inference component, the authors used a CNN-based approach to detect geometric primitives such as walls, doors, and windows from the input image. The detected primitives are then processed to infer their relationships, including their relative positions and orientations, using a combination of rule-based methods and learning-based methods. Specifically, the authors used a typology-based approach to model the layout and organization of geometric primitives in a building, which allows for the inference of relationships between primitives based on their functional and spatial relationships.
%
In the planar graph assembly component, the inferred primitives and their relationships are combined to form a planar graph that represents the 2D floor plan of the building. The authors used an integer programming approach to find the optimal planar graph that satisfies the inferred relationships between primitives, subject to certain constraints such as connectivity and planarity.
%
\par
Fuyang Zhang~\cite{zhang2021structured} proposed a novel approach for structured outdoor architecture reconstruction by exploration and classification, which leverages the power of heuristic actions, model classification, and iterative refinement to generate accurately. The method uses a combination of a heuristic-based exploration and a learning-based classification framework to improve the quality of the reconstructed models. The algorithm is designed to generate outdoor buildings structure with a high level of detail and accuracy, making it suitable for a range of applications in architecture, urban planning, and computer vision.
%
\par
Conv-MPN, proposed by Fuyang\etal~\cite{zhang2020conv}, is a novel message-passing neural network architecture that is used for reconstructing an outdoor building as a planar graph from a single RGB image. The goal of the network is to accurately identify the building edges in an image and represent them as nodes in the graph. The edges are then connected based on their relationships to create a structured representation of the building.
%
To train Conv-MPN, the authors used a two-stage process. In the first stage, a CNN is trained to predict the existence of edges in an image. The CNN is designed to output a binary mask that indicates the presence or absence of edges at each pixel location. In the second stage, Conv-MPN is trained to predict the structure of the building graph from the output of the CNN. This is done using a message-passing algorithm that iteratively refines the node features and edge connections until a stable graph structure is obtained.
%
\par
However, as a trade-off, Conv-MPN is computationally expensive due to its exhaustive search over the entire search space even based on some prior knowledge. This can limit its practical use in real-world scenarios, especially when dealing with large-scale and complex outdoor scenes. Nonetheless, with the increasing availability of powerful computing resources, Conv-MPN remains a promising approach for structured outdoor architecture reconstruction, especially in cases where accuracy is of utmost importance.
%
\par
\subsection{Purely DL Based}
Fully Deep Learning Based methods have shown great potential in achieving excellent results in boundary extraction for building images. One such method is LCNN, proposed by Zhou\etal, which stands for Line Segment Detection Convolutional Neural Network~\cite{zhou2019end}. The LCNN approach is a fully convolutional neural network that is designed to predict a set of line segments that represent the wireframe of an object in an input image.
%
The LCNN architecture consists of a backbone network for feature extraction and a series of prediction modules that predict line segments at different scales. The backbone network is composed of a series of convolutional layers followed by dilated convolutional layers that capture multi-scale contextual information. The prediction modules are then applied to the feature maps generated by the backbone network to predict line segments at different scales.
%

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{images/u2net.pdf}
    \caption{Schematic illustration of U2Net-Switch; the Left module is purely a U2Net model and the right module contains a sampler and classifier. The candidate edges are from the first four layers of U2Net not only the De\_1 layer.\textbf{( Note: U2Net is only for segmentation tasks, it can be replaced by any segmentation model, such as PSPNet~\cite{zhou2019fusion}, DeepLab v3~\cite{chen2017rethinking}, Transformer \cite{vaswani2017attention}, SETR
\cite{zheng2021rethinking},~\etc)}}
    
    \label{fig:overall}
\end{figure*}
%
The LCNN approach is trained end-to-end using a multi-task loss function that penalizes both false positives and false negatives in line segment detection while enforcing geometric constraints on the predicted line segments. By using this approach, LCNN achieves state-of-the-art performance on several benchmark datasets for wireframe parsing.
%
\par
Holistic Edge Attention Transformer (HEAT)~\cite{chen2022heat}is a deep learning-based method for the structured reconstruction of architectural floor plans from 2D images. One of the main contributions of HEAT is the introduction of a novel attention-based transformer architecture that is designed to capture the long-range dependencies and structural information in the input image.
%
HEAT adopts a more complex transformer architecture than ViT to handle the challenging task of structured reconstruction of floor plans. The proposed transformer architecture, called Holistic Edge Attention Transformer (HEAT), consists of three main components: edge attention, holistic attention, and edge fusion.
%
\par
In addition, it introduces a new loss function called Edge Map Loss (EML). EML is designed to penalize the predicted edges that deviate from the ground truth edges while ignoring the regions in the image that do not contain any edges. This loss function allows HEAT to focus on the important regions in the image and to produce more accurate edge maps for structured reconstruction.
\par
Meng \etal~\cite{meng2020lgnn} proposed Line Graph Convolutional Network(LGCN) for wireframe parsing from images. Wireframe parsing is the task of detecting and reconstructing the underlying wireframe structure of an object or a scene from an image. It is an important problem in computer vision, with applications in tasks such as object detection and recognition, and scene understanding.
%
Existing methods for wireframe parsing can be broadly categorized into two types: geometry-based methods and learning-based methods. Geometry-based methods rely on mathematical models and heuristics to detect and reconstruct wireframes from images. While these methods can achieve good accuracy in some cases, they are often limited in their ability to handle occlusions and incomplete wireframes. Learning-based methods, on the other hand, rely on deep learning models to learn the mapping between the input image and the corresponding wireframe. These methods have shown promising results in recent years, but they also suffer from limitations such as the need for large amounts of labeled data and the difficulty of handling occlusions and incomplete wireframes.
%
\par



